Searching for Regularity in Bounded Functions

Given a function $f$ on $\mathbb{F}_2^n$, we study the following problem. What is the largest affine subspace $\mathcal{U}$ such that when restricted to $\mathcal{U}$, all the non-trivial Fourier coefficients of $f$ are very small? For the natural class of bounded Fourier degree $d$ functions $f:\mathbb{F}_2^n \to [-1,1]$, we show that there exists an affine subspace of dimension at least $ \tilde\Omega(n^{1/d!}k^{-2})$, wherein all of $f$'s nontrivial Fourier coefficients become smaller than $ 2^{-k}$. To complement this result, we show the existence of degree $d$ functions with coefficients larger than $2^{-d\log n}$ when restricted to any affine subspace of dimension larger than $\Omega(dn^{1/(d-1)})$. In addition, we give explicit examples of functions with analogous but weaker properties. Along the way, we provide multiple characterizations of the Fourier coefficients of functions restricted to subspaces of $\mathbb{F}_2^n$ that may be useful in other contexts. Finally, we highlight applications and connections of our results to parity kill number and affine dispersers.

==> intro.tex <==
\section{Introduction}

The search for structure within large objects is an old one, and lies at the heart of Ramsey theory. 
For example, a famous corollary of Ramsey's theorem is that any graph on $n$ vertices must contain a clique or an independent set of size $\Omega(\log n)$. 
Another example is Van der Waerden's theorem \cite{vanderwaerden}\footnote{See also the more general Hales-Jewett theorem \cite{hales-jewett}.} which states for sufficiently large $n$, any coloring of $\{1,\ldots,n\}$ with $r$ colors must contain a monochromatic $k$-term arithmetic progression. 
Roth~\cite{roth} gave a similar result when they showed that \emph{every} subset of $\{1,\ldots,n\}$ of density $\delta > 0$ must contain a $3$-term arithmetic progression. 
%This result was later generalized by Szemer\'edi~\cite{szemeredi1975regular} to $k$-term arithmetic progressions.
% The existence of arithmetic progressions among subsets of integers is another example of this phenomenon. 
%In 1927, Van der Waerden~\cite{vanderwaerden} showed that for sufficiently large $n$, any coloring using $c$ colors of $\{1,\ldots,n\}$ must contain a monochromatic arithmetic progression of length $k$. 
% Roth~\cite{roth} in 1953, showed that for sufficiently large $n$, \emph{every} subset of $\{1,\ldots,n\}$ of density $\delta > 0$ must contain a $3$-term arithmetic progression. 
%Statements of this nature are not only deep mathematical discoveries, but have found many applications within theoretical computer science. For example, the Hales-Jewett Theorem~\cite{hales-jewett}, which implies Van der Waerden's theorem, was used to give the first nontrivial parallel repetition bounds for 2 player 1 round games~\cite{verbitsky}.
% In 1975, Szemer\'edi~\cite{szemeredi1975regular} generalized Roth's result for $3$-term arithmetic progressions to $k$-term arithmetic progressions. 
%A key ingredient in his work was the Szemer\'edi's Regularity Lemma for general graphs~\cite{szemeredi1975regular}, which showed that every graph on $n$ vertices can be partitioned into $k := M(\eps)$ parts $V_1 ,\ldots,V_{k}$, wherein most pairs of parts $(V_i, V_j)$ are ``$\eps$-regular". 
%We won't define what regularity formally means in this particular context but broadly speaking, one can think of it as saying that the bipartite graph induced across $V_i$ and $V_j$ appears as though the edges were sampled randomly. 
% Statements of this nature are not only deep mathematical discoveries, but have found many applications within theoretical computer science. 
Szemer\'edi's Regularity Lemma is also a well known example of this phenomenon. Roughly speaking, this lemma says that any graph $G$ can be partitioned into $k := M(\delta)$ parts $V_1 ,\ldots,V_{k}$, wherein most pairs of parts $(V_i, V_j)$ are $\delta$-regular. 
In this setting, $(V_i, V_j)$ being $\delta$-regular roughly corresponds to saying that the bipartite graph induced across $V_i$ and $V_j$ appears as though the edges were sampled randomly. This powerful statement has found applications in both pure mathematics (for example, Szemer\'edi~\cite{szemeredi1975regular} used it to generalize Roth's result for $3$-term arithmetic progressions to $k$-term arithmetic progressions) and theoretical computer science (the lemma has been used extensively in testing triangle freeness in dense graphs~\cite{ruzsa-szemeredi-triangles, triangle-freeness-dense}).

Inspired by Szemer\`edi's regularity lemma, Green \cite{green-regularity} gave an analogous regularity lemma for bounded functions of the form $f: \F_2^n\rightarrow [0,1]$. 
In order to state their result, we recall Fourier analysis over a subspace $\calV$ of $\F_2^n$. For a function $f:\calV \to \R$ we can write the Fourier decomposition $$f(x) = \sum_{\gamma \in \calV} \hat{f}(\gamma)\cdot \chi_\gamma(x),$$ where $\chi_\gamma: \calV \to \pmone$ is a character of $\calV$ and its corresponding Fourier coefficient is given by $\hat{f}(\gamma) = \E_{x \sim \calV}[f(x)\chi_\gamma(x)]$\footnote{For more on this powerful representation we refer the reader to \cite{AOBFbook}, and for details on Fourier analysis on subspaces, see \Cref{section:prelim}.}.
Furthermore, we need a definition of $\delta$-regularity for functions over $\F_2^n$.
\begin{definition}[$\delta$-regular\footnote{It is easy to check that when we sample $f : \F_2^n \to \{0,1\}$ to be a random Boolean function then with with extremely high probability it will be $2^{-\Omega(n)}$-regular (see \cite{AOBFbook}, Exercise 1.7 and Proposition 6.1). In this sense, being $\delta$-regular is a sort of pseudorandomness condition, analogous to the definition of $\delta$-regularity for graphs in Szemer\'edi's regularity lemma.}]
\label{def:delta-regular}
Let $f: \calV \to \R$. We say that $f$ is \emph{$\delta$-regular} if
$$\max_{\gamma \in \calV, \gamma \neq \mathbf 0}\abs{\hat{f}(\gamma)} \leq \delta.$$
\end{definition}

We can now state Green's result.
Below, we denote the restriction of a function $f$ to an affine subspace $\alpha + \calV$, as $f_{\alpha+\calV}$.
% \footnote{For more details on what we mean by restricting to an affine subspace, and how Fourier coefficients are affected due to such restrictions, see \Cref{section:prelim}.} 
The notation $\tower(x)$ refers to an exponential tower of 2's $2^{2^{\iddots}}$ of height $x$.

\begin{theorem}[Theorem 2.1 in \cite{green-regularity}\footnote{More precisely, an analogue of \Cref{thm:green-regularity} for $\{0,1\}$-valued functions is what actually appears in \cite{green-regularity}. However, the proof in \cite{green-regularity} follows just as well for functions taking values in $[0,1]$.}]
\label{thm:green-regularity}
Given any $f: \F_2^n \to [0,1]$, there exists some subspace $\calV \subseteq \F_2^n$ of co-dimension at most $M(\delta)$ such that $f_{\alpha + \calV}$ is $\delta$-regular for at least a $(1-\delta)$-fraction of all $\alpha$. Here, $M(\delta)\leq \tower(\ceil{1/\delta^3})$.
\end{theorem}

In the same paper, Green showed that $M(\delta) \geq \tower(\Omega(\log (1/\delta)))$ was necessary. Subsequently, Hosseini et al. \cite{hlms-regularity-lb} exhibited a better counterexample that showed co-dimension $M(\delta) \geq \tower(\ceil{1/16\delta})$ is required.

In the above upper and lower bound of \cite{green-regularity, hlms-regularity-lb}, note that the partition of $\F_2^n$ being chosen is of a very specific form -- namely it is simply every possible affine shift of a given subspace. Given this observation, one might wonder if there is a more clever partition of $\F_2^n$ into affine subspaces of higher dimension so that in most parts $f$ is $\delta$-regular.
%One might wonder if it is possible achieve better results via a more clever partition. 
This is indeed the case. 

\begin{proposition}[Proposition A.1 in \cite{ghz-simpler}\footnote{This is actually a simpler version of Proposition A.1 in \cite{ghz-simpler}, where we are not worried about multiple functions or conditioning on any events.}]
\label{claim:ghz-partition}

    There exists a partition $\Pi$ of $\F_2^n$, wherein every $\pi \in \Pi$ is an affine subspace of co-dimension at most $\frac{1}{\delta^3}$, such that $f$ is $\delta$-regular on at least $(1-\delta)$-fraction of the $\pi \in \Pi$. 

\end{proposition}

% He showed that one can partition $\F_2^n$ with affine shifts of a subspace $\calV$ so that the in most affine shifts, the restricted function is $\delta$-regular. Below, we denote the restriction of a function $f$ to an affine subspace $\alpha + \calV$, as $f_{\alpha+\calV}$.\footnote{For more details on what we mean by restricting to an affine subspace, and how Fourier coefficients are affected due to such restrictions, see \Cref{section:prelim}.} The notation $\tower(x)$ refers to an exponential tower of 2's $2^{2^{\iddots}}$ of height $x$.
%  key tool in testing triangle freeness in dense graphs~\cite{ruzsa-szemeredi-triangles, triangle-freeness-dense}. 
%Moreover, the ideas in the proofs of these theorems have also been used in other settings. 
%For example, a key idea in the recent proofs of the parallel repetition theorems for the GHZ game~\cite{ghz,ghz-simpler} crucially use ideas that are very similar to those in the proofs of Roth's theorem and the Regularity Lemma.

%The proofs of the above mentioned theorems have a common theme of repeatedly identifying structure in systems that do not resemble random objects. 
%We will briefly sketch how this is done in the setting of Roth's theorem. 
%We begin by noting that a randomly chosen set of $\{1,\ldots,n\}$ of a specific density, typically, has many $3$-term arithmetic progressions. 
%For example, in Roth's theorem, a key idea is that if a dense set $A$ does not contain $3$-term arithmetic progressions then it cannot resemble a randomly chosen set of the same density.
% This ``deviation" of $A$ from a random set is in turn used to find a sub-progression where $A$ is more dense.\footnote{Hence being known as a ``density increment" argument.}  
%
%
%We can use Fourier analysis to make this intuition precise. 
% order to reason about such differences between structured objects and random ones is Fourier analysis. 
%In particular, we can understand functions defined over Abelian groups by writing them as linear combinations of the characters of the group. 
%One can check that random functions\footnote{for example, the indicator function of random subset of the elements of the group}, typically, do not correlate with any non-trivial character.
%Roughly speaking, in Roth's theorem, when we say a set $A$ does not ``resemble" a random set of the same density, this corresponds to $\indicator_A$ having a large correlation with a non-trivial character.\footnote{In other words, $\indicator_A$ has a large Fourier coefficient.}
%Conversely, if $\indicator_A$ has small correlation with characters (i.e. it looks like a random set) it is not hard to show that it must have many arithmetic progressions.
%Moreover, in many cases, we can also use the correlation of a function with some character as a proxy for how far the function is from being ``random". 
%For example, in Roth's theorem, it turns out that if a set does not have any $3$-term arithmetic progressions then an appropriately chosen function must have a large correlation with some (non-trivial) character.

%This dichotomy between random objects and structured ones is also a key feature of the Szemer\'edi regularity lemma. Broadly speaking, it shows that every graph on $n$ vertices can be partitioned into $k := M(\delta)$ parts $V_1 ,\ldots,V_{k}$, wherein most pairs of parts $(V_i, V_j)$ are ``$\delta$-regular". 
%In this setting, $(V_i, V_j)$ being ``$\delta$-regular" roughly corresponds to saying that the bipartite graph induced across $V_i$ and $V_j$ appears as though the edges were sampled randomly. 

% We discuss its role in the proof of Roth's theorem briefly. For a function $f: \mathbb{Z}/N\mathbb{Z} \rightarrow \mathbb{C}$, one can write its Fourier transform as
% \begin{align*}
%     f(x) = \sum_{j= 0}^{N-1}\hat{f}(j)e^{(2\pi ij)/N},
% \end{align*}
% where $\hat{f}(j) := \E[f(x)e^{(-2\pi ij)/N}]$ is the Fourier coefficient of $f$ corresponding to the angle $2\pi j/N$. 
% For Roth's theorem one thinks of $A$ as a subset of the first $N = 2n+1$ natural numbers and considers the corresponding indicator function $\indicator_A : \mathbb{Z}/N\mathbb{Z} \to \{0, 1\}$. 
% It turns out that if $A$ does not contain $3$-term arithmetic progressions then $\indicator_A$ must have a large non-trivial Fourier coefficient which allows one to find a sub-progression on which $A$ is slightly denser. 
% In contrast, if $\indicator_A$ has small Fourier coefficients -- which is typically true if $A$ is chosen randomly -- then one can show that it must contain many 3-term arithmetic progressions. At a very high level, the proof of Szemer\'edi's Regularity Lemma follows a similar roadmap: one uses the existence of non-regularity within a partition to further subdivide the vertices into ``more regular" parts.

%One can also ask if such  
%\Snote{TODO: say a few lines here to discuss why it makes sense/is relevant to ask for a pseudorandom partition of $\F_2^n$ for functions} 
In this work, rather than searching for a partition wherein most parts are $\delta$-regular (as in \Cref{thm:green-regularity} or \Cref{claim:ghz-partition}), we instead look for a single affine subspace such that $f$ is $\delta$-regular. Namely, our main focus is to understand the following quantity:
% \begin{definition}[$\delta$-regularity number]
% \label{dfn:delta-regularity-number}
    % For a function $f:\F_2^n \rightarrow \R$ and $\delta > 0$, define the $\delta$-regularity number as
    $$\regnum(f,\delta) := \min\{\codim(\calV): \text{ for some } \alpha\in \F_2^n, f_{\alpha+\calV} \text{ is } \delta\text{-regular}\}.$$
% \end{definition}
% Every function $f: \F_2^n \to \R$ can be rewritten
%\footnote{For more on this powerful representation and how it has found use throughout theoretical computer science, we refer the reader to \cite{AOBFbook}.} 
% in the Fourier basis as
% $$f(x) = \sum_{\gamma \in \F_2^n} \hat{f}(\gamma)\cdot \chi_\gamma(x),$$
% where $\chi_{\gamma}$ is the character corresponding to the vector $\gamma$ and can be written as $\chi_\gamma(x) = (-1)^{\langle \gamma, x\rangle}$. 
% Moreover, the number $\hat{f}(\gamma)$ is referred to as the Fourier coefficient corresponding to $\gamma$ and is given by $\hat{f}(\gamma) = \E_x[f(x)(-1)^{\langle x,\gamma\rangle}]$. This representation has found several applications in mathematics and theoretical computer science. Some of the remarkable results in the study of Boolean functions, derived using Fourier analysis include,
% \begin{itemize}
%     \item[1.] sharp thresholds of monotone graph properties \cite{FK},
%     \item[2.] a result in social choice theory which says that fair, unbiased elections can be fixed, with good probability, by fixing at most $O(1/\log n)$ fraction of the votes \cite{KKL}, and,
%     \item[3.] lower bounds for various models of computation \cite{LMN93,Tal17} such as $\mathsf{AC}^0$ circuits, bounded depth decision trees, DNFs, etc.
% \end{itemize} 
% For more on this powerful representation we refer the reader to \cite{AOBFbook}.
% Inspired by the proof of Roth's theorem, we have the following definition of pseudorandomness.



%The extension of these ideas into the realm of functions over $\F_2^n$ is not new. 
%As in the classical proof of Roth's theorem, Fourier analysis will provide useful insights as to how ``regular" or ``pseudorandom" a function $f: \F_2^n \to \R$ is. It is well known\footnote{For more on this powerful representation and how it has found use throughout theoretical computer science, we refer the reader to \cite{AOBFbook}.} that any function $f: \F_2^n \to \R$ can be rewritten in the Fourier basis:
%$$f(x) = \sum_{\gamma \in \F_2^n} \hat{f}(\gamma)\cdot (-1)^{\inner{\gamma, x}},$$
%where $\hat{f}(\gamma) = \E_x[f(x)(-1)^{\langle x,\gamma\rangle}]$ is the Fourier coefficient of $f$ corresponding to $\gamma$.
%Inspired by the proof of Roth's theorem, we have the following definition of pseudorandomness.


%Like in Szemer\'edi's Regularity Lemma one can also if there is a partition of $\F_2^n$ into affine subspaces so that $f$ is $\delta$-regular in most parts. 
%We pause here to note that this definition of regularity can be easily extended to functions over general finite Abelian groups $f: G \to \R$, and indeed this matches exactly the notion of regularity in the proof of Roth's theorem.
%
%We again recall Szemer\'edi's regularity lemma, which, roughly speaking, says that one can partition any graph so that the induced bipartite graph across most parts appears psedudorandom. 
%Inspired by Szemer\'edi's Regularity Lemma, 
% A version of this question was considered by Green \cite{green-regularity} where he gave the following ``regularity" lemma for bounded functions of the form $f: \F_2^n\rightarrow [0,1]$. He showed that one can partition $\F_2^n$ with affine shifts of a subspace $\calV$ so that the in most affine shifts, the restricted function is $\delta$-regular. 



% One can further relax the condition of finding an affine partition and ask for even a \emph{single} affine subspace where the function is $\delta$-regular. 
% %, rather than a whole partition where most parts are good? 
% For a given function, can we find an affine subspace of co-dimension smaller than $\delta^{-3}$ where it is $\delta$-regular? This question motivates the following quantity that we seek to understand in this paper. 



A simple upper bound on $\regnum(f,\delta)$ for functions bounded in the interval $[-1,1]$ comes from the following folklore claim.

\begin{proposition}[Folklore]
    \label{claim:trivial-algorithm}
    For any $f : \F_2^n \to [-1,1]$ we have $\regnum(f,\delta) \leq \frac{1}{\delta}$.
\end{proposition}

The proofs of \cref{claim:ghz-partition} and \Cref{claim:trivial-algorithm} are based on simple algorithms that greedily fix the parities corresponding to the largest Fourier coefficients. Their proofs can be found in \Cref{appendix:omitted} for completeness.

\subparagraph*{Parity Kill Number.} Before detailing our results, it is worth mentioning the notion of parity kill number, which, in words, asks how many parities one has to fix in order to make a function $f$ over $\F_2^n$ constant.


\begin{definition}[Parity Kill Number]\label{def:paritykill}
We call the \emph{parity kill number} of a function $f: \F_2^n \to \pmone$ the minimum co-dimension affine subspace under which $f$ becomes a constant. The parity kill number, following \cite{parity-kill}, is denoted as $C_{\min}^{\oplus}[f]$. 
\end{definition}

We pause to note two things about this definition.
\begin{enumerate}
    \item The parity kill number of a function $C_{\min}^\oplus[f]$ can be seen as a generalization of the minimum certificate complexity $C_{\min}[f]$, and in particular we have the relationship $C_{\min}^\oplus[f] \leq C_{\min}[f]$ for all $f$.
    \item For any $f$ and $\delta > 0$, we have $\regnum(f,\delta)\leq C_{\min}^{\oplus}[f]$ since any subspace where $f$ is constant is automatically $\delta$-regular. Thus, a function's $\delta$-regularity number can be seen as a further generalization parity kill number.
    
\end{enumerate}

The parity kill number has been studied in several previous works. It was shown in \cite{parity-kill} that the parity kill number obeys a composition theorem.

\begin{theorem}[\cite{parity-kill}]
    \label{thm:parity-kill-composition}
    Let $f: \F_2^n \to \F_2$, and $g: \F_2^m \to \F_2$. We have that 
    $$\paritykill{f \circ g} \geq \paritykill{f} + C_{\min}[f]\cdot B_g,$$
    
    where $B_g = \max\{\log \paritykill{g} -1, 1\}$.
\end{theorem}
In fact, in \cite{parity-kill} \Cref{thm:parity-kill-composition} appeared as 
$$\paritykill{f \circ g} \geq \paritykill{f} + C_{\min}[f],$$
but they only assumed that $\paritykill{g} \geq 2.$ Therefore, the above result is strictly stronger for any $g$ such that $\paritykill{g}> 4$. We include a slightly simpler proof of this slightly stronger fact in \Cref{appendix:paritykill}. 

We mention (and improve slightly) \Cref{thm:parity-kill-composition} because it actually implies some of the strongest explicit functions that require large co-dimension to become $\delta$-regular. For a precise statement, see \Cref{claim:superlinear-boolean}.

\subparagraph*{Affine Dispersers and Extractors} Parity kill number and $\delta$-regularity number are intimately related to notions of affine dispersers, which have been well studied in the literature \cite{shaltiel-disperser, xinli-polylog-affine-dispersers, chattopadhyay-etal-affine-dispersers-logn, cohen-tal-f2polys}. 
\begin{definition}[Affine Disperser]
\label{dfn:affine-disperser}
    We say that a function $f:\F_2^n \to [C]$ is an \emph{affine disperser} if, for all affine subspaces $\calU$ of dimension at least $k$, it holds that $f_\calU$ is nonconstant.\footnote{Affine dispersers are sometimes alternatively defined as requiring that $\supp(f_\calU) \geq (1-\eps)C$ for some parameter $\eps$. Sometimes the output space is also alternatively defined as $\{0,1\}^m$ for some $m$ (see e.g. \cite{shaltiel-disperser, xinli-polylog-affine-dispersers, chattopadhyay-etal-affine-dispersers-logn}) or $\F_q$ for some (prime power) $q$ (see e.g. \cite{cohen-tal-f2polys}).}  
\end{definition}

In particular, as pointed out in \cite{parity-kill} when $C = 1$, an affine disperser for dimension $k$ is simply a function $f:\F_2^n \to \{0,1\}$ such that $\paritykill{f} \geq n - k - 1$.
 Cohen and Tal~\cite{cohen-tal-f2polys} showed that low-degree $\F_2$-polynomials would not make good affine dispersers. 
\begin{theorem}[\cite{cohen-tal-f2polys}]
\label{thm:cohen-tal}

If $f$ is degree-$d$ as an $\F_2$ polynomial, then for all $d\leq \log(n)/10$ there exists a dimension $k = \Omega(d\cdot n^{1/(d-1)})$ affine subspace $\calU$ in which $f$ becomes constant.

\end{theorem}
 We pause to note that the $\F_2$ polynomial representation of function over $\F_2$ possesses entirely different structure than the Fourier polynomial representation, which is the representation we work with in this writeup. 
 
Affine dispersers are a more relaxed version of affine extractors, which are functions that are required to look pseudorandom on large affine subsapces rather than just nonconstant.

\begin{definition}[Affine Extractor]
\label{dfn:affine-extractor}
A function $f:\F_2^n \to [C]$ is said to be a $(k, \delta)$-\emph{affine extractor} if for all affine subspaces $\calU$ of dimension at least $k$, we have that $$TV(f_\calU, \uniform_C) \leq \delta,$$
where $TV(\cdot,\cdot )$ is the statistical distance and $\uniform_C$ is the uniform distribution over $[C]$.
\end{definition}

Our notion of $\delta$-regularity number is closely related to affine extractors in the following sense. 
Suppose $f$ is a $(k, \delta)$-affine extractor. 
Then we claim that that $\regnum(f, \delta) \leq n - k -1$, or in other words that $f$ is $\delta$-regular on at least one subspace of dimension $k+1$. Indeed, suppose not. 
Then for all affine subspaces of dimension $k+1$ we have that $f$ has a Fourier coefficient which is larger than $\delta$. Let $\calU$ be one of these subspaces, and suppose without loss of generality that $\hat{f_{\calU}}(\mathbf 0) \geq 0$ and $\hat{f_\calU}(\gamma) > \delta$. Then we can fix the parity corresponding to $\gamma$, giving us a new affine subspace $\tilde \calU$ of dimension $k$ such that $\hat{f_{\tilde \calU}}(\mathbf{0}) = \hat{f_\calU}(\mathbf{0}) + \hat{f_\calU}(\gamma) > \delta$,\footnote{For details on why this equation holds, see \Cref{cor:V-dim-n-1}.} which is a contradiction.



\subsection{Our Results}

This line of work and questions lead directly to our main focus: for a general function $f$ can we obtain upper bounds better than~\Cref{claim:trivial-algorithm} on $\regnum(f,\delta)$? 
What are the best bounds that we can hope to achieve? 
We focus on the case when the output $f$ is either bounded in the interval $[-1,1]$ or it takes one of two values $\{-1,1\}$. 
Our first result is an upper bound on $\regnum(f,\delta)$ for functions with Fourier degree at most $d$ i.e. functions whose Fourier coefficients are all supported on vectors of weight at most $d$.

\begin{thm}[Upper bound on $\regnum(f,\delta)$ for degree $d$ bounded functions]
    \label{thm:bounded-deg-d-upper-bound-intro}
    For $\delta\in (0,1)$ and any degree $d$ function $f:\F_2^n \to [-1,1]$, there exists an affine subspace $\calU$ of dimension $\Omega\left(n^{1/d!}\left(\log(n/\delta) + d\right)^{-2}\right)$ such that $f_{\calU}$ is $\delta$-regular. In other words, we have 
    $\regnum(f,\delta) \leq n - \tilde{\Omega}\left( n^{1/d!}\right)$.
\end{thm}
% \Snote{the dependence of $\delta$ is missing in the thm statement, which might be worth including?}
We emphasize that, for small $d$, the most important factor in the above is the $n^{1/d!}$. We give a proof sketch of \Cref{thm:bounded-deg-d-upper-bound-intro} in \Cref{subsec:pf-sketch-thm}.
A consequence of \Cref{thm:bounded-deg-d-upper-bound-intro} is a lower bound on the dimension of low degree affine dispersers (see \Cref{cor:rule-out-dispersers}).
The lower bound on the dimension is obtained by studying the Fourier spectrum of ``$G$-granular" functions -- functions whose output is always an integer multiple of $G$ (see \Cref{def:granular-fn}).  
The main idea behind the proof is that a low degree affine disperser $f:\F_2^n\to[C]$ can be used to obtain a low degree function $h$ that is bounded in the interval $[-1,1]$, and in addition is $2/C$-granular.
It turns out that the Fourier coefficients of granular functions are also ``granular" (see \Cref{claim:granular-coefficients}) albeit with a different granularity and this feature is crucially used to argue that for an appropriate choice of $\delta$, if the function is $\delta$-regular then in fact it must be constant.
%It turns out that the Fourier coefficients of degree $d$, $G$-granular functions are also granular, in particular, they are always integer multiples of $2^{-d+1}\cdot C^{-1}$ (see \Cref{claim:granular-coefficients}). 

To complement this result, we also give several examples of functions (some bounded, some Boolean, some explicit, some existential) which are not $\delta$-regular in any subspace of small co-dimension. In other words, these functions have a large $\delta$-regularity number. This is summarized in the \Cref{table:large-reg-nums}.

\begin{table}[h!]
\centering
\begin{tabular}{||c | c | c | c | c ||} 
 \hline
 $\delta$ & $\regnum(f,\delta) \geq$ & Explicit? & Boolean/bounded & Ref. \\ 
 [0.5ex] 
 \hline\hline \rule{0pt}{3ex}  
  $1/n$ & $n/2 - 1$ & Yes & bounded & \Cref{claim:degree-one-bounded-lb}\\
 $\binom{n}{d}^{-1}$ & $n - 2dn^{1/(d-1)}$ & No & bounded & \Cref{claim:degree-d-bounded-lb} \\
 $\Theta(n^{-1/2})$ & $\Theta(\sqrt{n})$ & Yes & Boolean &  \Cref{lemma:majority-lower-bound}  \\ 
 $1/2^{2^k + 1}$ (for integer $k$) & $\Omega\left ((\log\frac{1}{\delta})^{\log_2(3)}\right )$ & Yes & Boolean & \Cref{claim:superlinear-boolean} \\
 $\frac{1}{2}\cdot n^{-d}$ (for $d \leq \frac{\log n}{\log \log n + 1}$) & $n - 2dn^{1/(d-1)}$ & No & Boolean & \Cref{cor:nonexplicit-boolean-simpler} \\
 [0.5ex] 
 \hline
\end{tabular}
\caption{Table of functions with large $\delta$-regularity numbers.}
\label{table:large-reg-nums}
\end{table}


% \Mnote{TODO: remarks on the above table}



We comment now briefly on each of the entries in \Cref{table:large-reg-nums}.


\subparagraph*{Bounded Lower Bounds.}

\Cref{claim:degree-one-bounded-lb} is based on the simple degree one function $f(x) = \frac{1}{n}\cdot \sum_i (-1)^{x_i}$. A simple argument (see \Cref{claim:std-basis-vecs-in-small-subspace}) shows that in any subspace of dimension larger than $n/2$, there must exist a Fourier coefficient that has only one old standard basis vector ``falling" to it. This immediately implies \Cref{claim:degree-one-bounded-lb}.

\Cref{claim:degree-d-bounded-lb} is based on a random homogeneous degree $d$ function $f_\bfz(x) = \binom{n}{d}^{-1}\sum_{\gamma: \norm{\gamma}_1 = d}\bfz_\gamma(-1)^{\inner{\gamma, x}}$, where $\bfz_\gamma \sim \pmone$ is a random sign. At a high level, we show that in any sufficiently large affine subspace $\alpha + \calV$ there must be many nonempty cosets of $\calV^\perp$ that contain weight $d$ vectors. Since via \Cref{fact:Fourier-coeff-of f_U-as-a-sum-of-fourier-coeff-of-f-from-vperp} these cosets correspond to Fourier coefficients of the restricted function, it must be that they cancel nicely. We show that this happens with very small probability over the choice of our random function.

\subparagraph*{Boolean Lower Bounds.}
\Cref{lemma:majority-lower-bound} is based on the majority function, and is tight for the majority. One way to try and make majority have small Fourier coefficients is to fix more and more bits to the same value. \Cref{lemma:majority-lower-bound} shows that this is indeed an optimal strategy. We remark that \Cref{lemma:majority-lower-bound} also gives an explicit example wherein the trivial algorithm given by \cref{claim:trivial-algorithm} is optimal for $\delta = \Theta(n^{-1/2})$.

\Cref{claim:superlinear-boolean} is based on a simple function $f$ on 4 inputs that is composed with itself $k$ times. The function itself is actually the same one as was considered in \cite{parity-kill}, and indeed we use their main theorem (\Cref{thm:parity-kill-composition}) crucially to obtain our lower bound. At a high level, we show that
\begin{enumerate}
    \item $f$ has a minimum certificate complexity of 3, which by \Cref{thm:parity-kill-composition} means that $f^{\circ k}$ has a parity kill number of at least $3^{k-1}$, and
    \item that $f^{\circ k}$ is degree $2^k$, and therefore its Fourier coefficients are all multiples of $1/2^{2^k}$.
\end{enumerate}  
By the second point, in order to make all the Fourier coefficients smaller than $1/2^{2^k}$, we must actually make $f$ constant. Combining these two points yields \Cref{claim:superlinear-boolean}.

One might hope that, to complement the lower bounds of \Cref{lemma:majority-lower-bound} and \Cref{claim:superlinear-boolean}, we have an upper bound for Boolean functions along the lines of $\regnum(f,\delta) \leq \sqrt{n}\cdot \polylog(1/\delta)$.
\Cref{cor:nonexplicit-boolean-simpler} rules this out strongly. Its major downside is that it is not explicit. 
An interesting open problem would be to exhibit an explicit Boolean function that exhibits a similarly strong lower bound on the regularity number. 
The proof of \Cref{cor:nonexplicit-boolean-simpler} is based on a simple lemma of \cite{hlms-regularity-lb} (\Cref{lemma:bounded-regularity-to-boolean-regularity}), which uses the probabilistic method to show the existence of a Boolean function whose Fourier coefficients are extremely close to those of the bounded function on all sufficiently large affine subspaces. We can therefore apply \Cref{lemma:bounded-regularity-to-boolean-regularity} to the lower bound from \Cref{claim:degree-d-bounded-lb} to achieve the result.
We also note that the Boolean function counterexamples are examples of dispersers whose output is $\{0,1\}$ and stronger, explicit counterexamples will yield explicit dispersers with better parameters.

\begin{remark}
The lower bound for bounded functions in \Cref{claim:degree-d-bounded-lb} is a degree $d$ function, and as we discussed we use \Cref{lemma:bounded-regularity-to-boolean-regularity} to convert it to a Boolean function. 
%Moreover, all the non-zero Fourier coefficients of the bounded, degree $d$ function have magnitude $\binom{n}{d}^{-1}$. 
Although the magnitude of the Fourier coefficients of the corresponding Boolean functions are very close to those of the bounded ones, these functions are quite far from being low degree. Indeed, since all the low degree Fourier coefficients are close to $\binom{n}{d}^{-1}$ in magnitude, there is roughly $1-\binom{n}{d}^{-1}$ mass on the Fourier coefficients of degree larger than $d$.
\end{remark} 

% \Mnote{Some sort of remark (perhaps put elsewhere) that the Fourier coefficients look similar, but the boolean function actually cannot be too close to degree $d$.}

% \Mnote{TODO: discuss Boolean vs bounded degree $d$}

\subparagraph*{Boolean Degree $d$ Functions.} From the above discussion, it is clear that we cannot hope to obtain strong upper bounds on $\regnum(f,\delta)$ in general. 
However, it is true that degree $d$ Boolean functions have much smaller regularity numbers than what can be said for bounded functions. 
Boolean degree $d$ functions have been extensively studied, and it is well-known (see e.g. \cite{buhrman-dewolf-boolean-fn-complexity}) that the degree $d$ of a Boolean function and its certificate complexity are polynomially related. 
In particular, Midrijanis~\cite{Midrijanis-degree-certificate-cxty} showed the following.
\begin{lemma}[\cite{Midrijanis-degree-certificate-cxty}]
\label{claim:midrijanis}
For any $f:\{0,1\}^n \to \{0,1\}$ we have that $D(f) \leq 2\cdot \deg(f)^3$, where $D(\cdot)$ denotes the decision tree complexity of $f$.
\end{lemma}
% that $C[f]\leq 2\cdot \deg(f)^3$. 
This gives a much stronger result for Boolean degree $d$ functions than our corresponding result for bounded degree $d$ functions. Namely, we have the following.
\begin{claim}
For any degree $d$ function $f: \F_2^n: \to \pmone$, it holds that $\regnum(f,\delta) \leq 2d^3$ for all $\delta \geq 0$.
\end{claim}
\begin{proof}
The result follows from \Cref{claim:midrijanis} and via the observation that $\regnum(f,\delta) \leq \paritykill{f}\leq C_{\min}[f] \leq C[f] \leq D(f)$.
\end{proof}

A key idea in the proof of \Cref{claim:midrijanis} is a clever application of Markov's theorem. 
One might hope to obtain stronger bounds on the dimension for low degree affine dispersers via this argument.
Indeed, a slight modification of this idea shows that degree $d$ functions $f:\F_2^n \to[C]$ have certificate complexity $O(Cd^3)$. However, this does not say anything non-trivial if $C \gg n/d^3$. On the other hand, \Cref{cor:rule-out-dispersers} still gives meaningful results if $C$ is large. 

\subsection{Proof Sketch of \Cref{thm:bounded-deg-d-upper-bound-intro}}
\label{subsec:pf-sketch-thm}
We give a brief proof sketch of~\Cref{thm:bounded-deg-d-upper-bound-intro}. While there are certainly details to work through, the heart of the proof comes down to a pigeonhole principle argument.
The proof proceeds by induction over the Fourier degree. We start with the base case corresponding degree one functions, where we can assume that our function has the form 
$$f(x) = \hat{f}(0) + \sum_i \hat{f}({e_i})\chi_{e_i}(x).$$ 

For a parameter $t \geq 1$ and a subset $S\subseteq [t]$ consider the sum $g_S = \hat{f}(0) + \sum_{i \in S}\hat{f}(e_i)$. Note that $g_S = \E[f(x) | x_i = 0 \:\: \forall i \in S] \in [-1,1]$. 
Therefore, the pigeonhole principle tells us that if we set $t = \Omega(\log 1/\delta)$ there must exist two distinct sets $S,S'$ such that the difference $|g_S - g_{S'}| \leq \delta$. 
We can further write $g_S - g_{S'} = \sum_{i\in S\triangle S'}\hat{f}(e_i)(-1)^{|\{i\}\cap S'|}$.  We will now use the set $S\triangle S'$ and the signs to construct an affine subspace where at least one Fourier coefficient will have small magnitude. 

Assume without loss of generality that $1\in S\setminus S'$ and $S\triangle S' = [t']$ for some $t'\leq t$.
Let us now  restrict ourselves to the affine subspace $\calU$ given by the linear equations $x_1 + x_i = b_i$, for each $i\in \{2,\ldots,t'\}$ and $b_i = |\{i\}\cap S'|$. 
We can reason about the Fourier spectrum of $f_\calU$ by simply plugging in $x_{i} = b_i + x_{1}$.
Under this restriction we see that the Fourier coefficients of $e_{t'+1},\ldots,e_n$ remain unchanged and the new Fourier coefficient of $e_1$ is exactly equal to 
$$\hat{f}(e_{1}) + \sum_{i = 2}^{t'} \hat{f}({e_i})(-1)^{b_i} = g_S - g_{S'},$$
which we observed has magnitude at most $\delta$. We can now repeatedly apply this argument roughly $\frac{n}{\log(1/\delta)}$ times for the remaining standard basis vectors corresponding to large Fourier coefficients.
At the end of this process, when we run out of standard basis vectors for the pigeonhole principle, we can fix the coordinates corresponding to any large coefficients that remain arbitrarily to obtain a $\delta$-regular function on a subspace of dimension $\Omega\left(\frac{n}{\log(1/\delta)}\right)$.


At a high level, we will reduce the problem for degree $d$ functions to degree $d-1$ by ensuring that under an appropriately chosen affine subspace -- whose dimension is at least $\tilde{\Omega}(n^{1/d})$ -- the restricted function is degree $d$ and all the Fourier coefficients at the $d$-th level are extremely small $\ll \delta/n^d$. For a detailed statement, see \Cref{lemma:degree-d-small}. 
The last constraint ensures that when we use the inductive hypothesis for $d-1$ the degree $d$ coefficients do not disturb the new coefficients even if they combine in the most constructive way possible. 

This is done by repeatedly applying the pigeonhole principle again, however, the key issue that we must address is that unlike the degree one case, several Fourier coefficients could get affected when we apply a restriction. In order to deal with this, we apply restrictions in an iterative manner so that each iteration preserves the small Fourier coefficients from past iterations while still making sure that \emph{several} new Fourier coefficients are additionally small. The price we pay for this is that in each iteration we apply the pigeonhole principle using larger and larger subsets of the standard basis vectors.



==> prelim.tex <==
\section{Preliminaries}
\label{section:prelim}
\subparagraph*{Notation.} 
$\indicator\{ \cdot\}$ denotes the an indicator function, which takes the value 1 if the clause is satisfied and 0 otherwise.
For a set $J\subseteq [n]$, we will use $\spn(J)$ to denote the subspace spanned by the standard basis vectors corresponding to the elements in  $J$.
For subsets $S \subseteq \F_2^n$, we denote $S^{=t} := S \cap \{u : \norm{u}_1 = t\}$.
We will refer to the $\text{L}_1$ norm of $\gamma \in \F_2^n$ by $\|\gamma\|_1$. Further, we define the degree of a function $f:\F_2^n \rightarrow \R$ to be $\max\{\|\gamma\|_1: \hat{f}(\gamma) \neq 0\}$.
At several points, it will be useful for us to consider the compositions of functions with linear maps. For a function $f$ and a map $M: \F_2^n \rightarrow \F_2^n$, we denote by $f\circ M$ the composition of the functions $f$ with $M$. In particular, $f\circ M(x)= f(M(x))$. 

\subparagraph*{Linear Algebra.} We will frequently interpret a linear transformation $M:\F_2^n\to\F_2^n$ as a matrix and refer to the linear map obtained by taking the transpose of the matrix as $M^{\transpose}$. The following fact about the action of $M$ and $M^{\transpose}$ on subspaces of $\F_2^n$ will be useful for us. 

\begin{fact}
\label{fact:orthogonal-subspace-transformation}
Suppose $M : \F_2^n \to \F_2^n$ is an invertible linear transformation and $A, B \subseteq \F_2^n$ are subspaces. If $MA:= \{Ma:a\in A\} = B$ then $M^\transpose B^\perp := \{M^{\transpose}b: b\in B^{\perp}\} = A^{\perp}$.
%
%Moreover, this implies that if $M$ is invertible, then $M^{-\transpose}$ maps $A^\perp$ to $B^\perp$.
\end{fact}
\begin{proof}
Let $u \in B^\perp$ and $a \in A$. Then we have that $\inner{M^{\transpose}u, a} = \inner{u, M a}$ which equals $\inner{u, b} = 0$ for some $b \in B$. This shows that $M^\transpose B^\perp \subseteq A^\perp$.

Next, for any $b \in B$ and $v\in A^{\perp}$ we have $\inner{M^{-\transpose}v , b} = \inner{v,M^{-1}b}  = 0$, as $M^{-1}b\in A$. This implies that $M^{-\transpose} v \in B^\perp$ which implies $v \in M^{\transpose} B^\perp$, so $A^\perp \subseteq M^{\transpose} B^\perp$ and we have equality.
\end{proof}

The notion of complement subspace will be useful for us. We say two subspaces $\calV,\calW$ of $\F_2^n$ are complements of each other, if every vector $x\in\F_2^n$ can be expressed uniquely as $v+w$ for $v\in\calV$ and $w\in \calW$.

\begin{fact}
\label{fact:cosets-unique}
Let $A$ be a subspace of $\F_2^n$ and $B$ be a complement subspace, so that $A \oplus B = \F_2^n$. Then for all distinct $b , b' \in B $, the cosets $b + A$ and $b' + A$ are mutually disjoint.
\end{fact}

\begin{proof}
Suppose not. Then we have that $b + a = b' + a'$ for some $a,a' \in A$. But then this implies $b + b' \in A$, which can only happen if $b = b'$ since $A \cap B = \emptyset$ by definition of the complement.
\end{proof}

\subparagraph*{Fourier Analysis.} 
%  We already discussed the Fourier decomposition of functions over $F_2^n$ in the introduction. 
% More generally, let $\calV$ be a subspace of $\F_2^n$. We start by recalling the Fourier decomposition of functions $f:\calV\rightarrow \R$. Denote by $\hat{\calV}$ the set of characters of $\calV$ when $\calV$ is viewed as a group under the addition operation. We can write the function $f$ as 
% $$f(x) = \sum_{\chi \in \hat{\calV}}\hat{f}(\chi)\chi(x),$$
% where $\hat{f}(\chi) = \E_x[f(x)\chi(x)]$ and is referred to as the Fourier coefficient corresponding to the character $\chi$. 
% The set of characters forms a group under multiplication, which is isomorphic to the additive group of $\calV$. 
% Therefore, we can identify characters with elements of the group, and in particular, 
For $f:\F_2^n \to \R$, we can write $f$ in the Fourier basis as 
$$f(x) = \sum_{\gamma \in \F_2^n}\hat{f}(\chi_\gamma)\chi_\gamma(x),$$
where the $\{\chi_\gamma\}_{\gamma \in \F_2^n}$ are such that $\chi_\gamma(x) = (-1)^{\langle \gamma,x\rangle}$. $\{\chi_\gamma\}_{\gamma \in \F_2^n}$ are characters that form a basis for the dual group $\hat{\F_2^n}$, and have the property that $\E[\chi_\gamma(x)] = \indicator\{\gamma = \bf 0\}$. For shorthand, we will refer to $\hat{f}(\chi_\gamma)$ as simply $\hat{f}(\gamma)$. 
% In this notation, we can write every function $f:\F_2 ^n \rightarrow \R$ as 
% $$f(x) = \sum_{\gamma\in \F_2^n}\hat{f}(\gamma) \chi_{\gamma}(x).$$ 
We denote $f^{=d} (x):= \sum_{\norm{\gamma}_1 = d} \hat{f}(\gamma)\chi_\gamma(x)$ as the ``degree $d$'' part of $f$. For more on this topic, see \cite{AOBFbook}, which uses notation consistent with ours. 

\subparagraph*{Restrictions.} We will be concerned with understanding the Fourier coefficients of a function when it is restricted to some affine subspace of $\F_2^n$. In the special case when the coordinates in a set $J\subseteq [n]$ are fixed using the vector $b\in \F_2^J$, we will denote the restriction of $f$ thus obtained as the function $\Restricted{f}{J}{b} : \spn(\overline{J}) \rightarrow \R$ which can be written as $\Restricted{f}{J}{b}(x) = f(x+b).$
% For convenience and brevity, whenever it is clear from the context, we will use $b$ to denote the vector $\sum_{j\in J}b_je_j$.
Next, we recall the formula of the Fourier coefficients of the restricted function. Note that since the function is defined on $\spn(\overline{J})$ which is isomorphic to $\F_2 ^{\overline{J}}$, the character corresponding to $\gamma\in \spn(\overline{J})$ can simply be identified as $\chi_\gamma(x) = (-1)^{\langle\gamma,x\rangle}$.


\begin{fact}[Fourier Coefficients of Restricted Functions (see e.g. \cite{AOBFbook}, Proposition 3.21)]
\label{fact:fourier-coeffs-restricted}
For every $\gamma\in \spn(\overline{J})$ and $b \in \spn(J)$,
\[\hat{\Restricted{f}{J}{b}}(\gamma) =
\sum_{\beta \in \spn(J)} \hat{f}(\beta + \gamma)\chi_{\beta}(b).
\]
\end{fact}
%\begin{proof}\Mnote{omit?}
%We recall that 
%$\hat{\Restricted{f}{J}{b}}(\gamma) = \E[\Restricted{f}{J}{b}(x)\chi_\gamma(x)]$ and we can write
%$$\E[\Restricted{f}{J}{b}(x)\chi_\gamma(x)] = \E[f(x+b)\chi_\gamma(x)] = \E\left[\sum_{\gamma' \in \F_2^n}\hat{f}(\gamma')\chi_{\gamma'}(x+b)\chi_\gamma(x)\right] = \E\left[\sum_{\gamma' \in \F_2^n}\hat{f}(\gamma')\chi_{\gamma' +\gamma}(x)\chi_{\gamma'}(b)\right].$$
%Since $\E[\chi_{\gamma+\gamma'}(x)] = 1$ if $\gamma' + \gamma \in \spn(J)$ and zero otherwise, we have that 
%$$\hat{\Restricted{f}{J}{b}}(\gamma) = \sum_{\beta\in \spn(J)}\hat{f}(\gamma +\beta)\chi_{\gamma+\beta}(b) = \sum_{\beta\in \spn(J)}\hat{f}(\gamma +\beta)\chi_{\beta}(b),$$
%since $\chi_\gamma(b) = (-1)^{\langle b,\gamma\rangle} = 0$ as $b\in \spn(J)$ but $\gamma \in \spn(\overline{J})$.
%\end{proof}
\subsection{Fourier Analysis on Subspaces}
Now we move to the general setting of restricting functions to arbitrary affine subspaces. 
Let $\calU = \calV + \alpha$ be an affine subspace of $\F_2^n$. By the restriction of $f$ to $\calU$, we mean the function $f_\calU: \calV\rightarrow \R$ defined as $$f_\calU(x) = f(x+\alpha).$$ 

Suppose the dimension of $\calV$ is $k$. Let $\calW$ be any complement subspace of $\calV^\perp$.\footnote{Note that $\calV$ is not necessarily a valid choice for $\calW$.} For each element $\gamma\in \calW$, define the character $\chi_\gamma: \calV\to \pmone$ as $\chi_\gamma(x) = (-1)^{\inner{\gamma,x}}$ -- it is simply the canonical character of $\gamma$ in $\F_2^n$, restricted to $\calV$. It is easy to verify the following fact.
\begin{fact}
    \label{fact:W-gives-characters}
    For any complement subspace $\calW$ of $\calV^\perp$, we have that $\{\chi_\gamma: \gamma\in \calW\}$ is the character group $\hat{\calV}$.
\end{fact}
  
Using \Cref{fact:W-gives-characters} we show a simple formula for the Fourier coefficients of $f_{\alpha + \calV}$. 
\begin{fact}
\label{fact:coefficients-as-expectation}
Let $\calW$ be a complement to $\calV^\perp$. There exists an isomorphism $R: \hat{\calV} \to \calW$ such that 
$$\hat{f_{\alpha + \calV}}(\chi) = (-1)^{\inner{R\rchi, \alpha}}\E_{x \in \alpha + \calV}[f(x)(-1)^{\inner{R\rchi, x}}].$$
\end{fact}

\begin{proof}
 Via \Cref{fact:W-gives-characters}, we can write $\hat\calV = \{\chi_\gamma: \gamma \in \calW\}$. This gives a natural isomorphism  $R: \hat{\calV} \to \calW$, where $R\rchi_\gamma = \gamma$ so that $\chi_\gamma(x) = (-1)^{\inner{\gamma,x}}$, for each $x\in\calV$. By definition, the Fourier coefficient corresponding to $\chi$ of $f_{\alpha+\calV}$ is
$$\hat{f_{\alpha + \calV}}(\chi) = \E_{x\in \calV}[f(\alpha+x)\chi(x)] = \E_{x\in \calV}[f(\alpha+x)(-1)^{\inner{R\rchi,x}}] = (-1)^{\inner{R\rchi,\alpha}}\E_{x\in \calU}[f(x)(-1)^{\inner{R\rchi,x}}].$$
\end{proof}

\Cref{fact:choice-for-W} represents a simple and analogous formula for Fourier coefficients of functions restricted to affine subspaces, and we find it useful primarily in the proof of \Cref{lemma:bounded-regularity-to-boolean-regularity}.
We now present two additional ways of viewing the Fourier coefficients of $f_{\alpha + \calV}$, each of which we will find useful in different contexts. %In both ways, we make use of the following more explicit definition of $\calW$. 

\begin{fact}
\label{fact:choice-for-W}
    Let $\calV$ be a subspace of dimension $k$ and $\Gamma=\{\gamma_1,\ldots,\gamma_n\}$ be a basis of $\F_2^n$ so that the first $k$ vectors of $\Gamma$ span $\calV$. For any invertible linear transformation $M$ that maps $e_i$ to $\gamma_i$ for all $i \in k$, the subspace $\calW = \{M^{-\transpose} \gamma: \gamma \in \spn([k])\}$ is a valid choice for a complement subspace for $\calV^\perp$.
\end{fact}
\begin{proof}
Since $\spn([k])$ and $\spn(\overline{[k]})$ are complements of each other and $M$ is invertible it follows that $\calW = \{M^{-\transpose}\gamma:\gamma\in\spn([k])\}$ is a complement space for $\{M^{-\transpose}\gamma:\gamma\in\spn(\overline{[k]})\}$. Now using
\Cref{fact:orthogonal-subspace-transformation} for $M^{-1}$ we see that 
$$\{M^{-\transpose}\gamma:\gamma\in\spn(\overline{[k]})\} = \{M^{-\transpose}\gamma:\gamma\in\spn([k])^\perp\} =  \calV^{\perp},$$
which follows by setting $A = \spn([k])$ and $B = \calV$.
\end{proof}



% \subparagraph*{Fourier Coefficients of $f_{\alpha + \calV}$ as Fourier Coefficients of $\Restricted{f\circ M}{\overline{[k]}}{b}$.} 
Next, we show that the Fourier coefficients of a function restricted to an affine subspace are the same as the Fourier coefficients of the function $f \circ M$ under a suitable (normal) restriction, and for a particular choice of $M$.

\begin{fact}
\label{fact:affine-subspace-same-as-linear-transformation-with-restriction}
Let $M$ and the characters for $\hat \calV$ be as discussed in \Cref{fact:choice-for-W}. Denote $g := f\circ M$. For any affine subspace $\alpha  + \calV$, we have that 
$$\hat{f_{\calU}}(\chi) = (-1)^{\inner{b_1,T\rchi}}\cdot\hat{\Restricted{g}{\overline{[k]}}{b_2}}(T\rchi),$$
where $b_2 \in \spn(\overline{[k]})$, $b_1 \in \spn([k])$ such that $M^{-1}\alpha = b_1 + b_2$ and $T:\hat \calV \to \spn([k])$ is an isomorphism.
\end{fact}

\begin{proof}
Suppose $M^{-1} \alpha = b_1 + b_2$, where $b_1 \in \spn([k])$ and $b_2 \in \spn(\overline{[k]})$. Combining \Cref{fact:choice-for-W} and \Cref{fact:coefficients-as-expectation} we get an invertible linear transformation $R:\hat{\calV}\to \{M^{-\transpose}\gamma:\gamma\in \spn([k])\}$, and setting $R\rchi := M^{-\transpose}\gamma$ for some vector $\gamma\in \spn([k])$, we can write,
\begin{align}\label{eq:fourier-coeff-affine-subspace-to-std-restriction}
\hat{f_\calU}(\chi) = (-1)^{\inner{M^{-\transpose}\gamma,\alpha}}\E_{x\in \calU}\left[f(x)(-1)^{\langle M^{-\transpose}\gamma, x\rangle}\right]  
    &= (-1)^{\inner{\gamma,M^{-1}\alpha}}\E_{y\in b_2 +\spn([k])}\left[f(My)(-1)^{\inner{M^{-\transpose}\gamma, My}}\right] \nonumber \\ 
    &= (-1)^{\inner{\gamma,b_1+b_2}}\E_{z\in \spn([k])}\left[f\circ M(z + b_2)(-1)^{\inner{\gamma, z+b_2}}\right] \nonumber \\ 
    &= (-1)^{\inner{\gamma, b_1}}\cdot \hat{\Restricted{g}{\overline{[k]}}{b_2}}(\gamma). 
\end{align}
The claim follows by setting $T = M^{\transpose}\circ R$. 
\end{proof}
\Cref{fact:affine-subspace-same-as-linear-transformation-with-restriction} implies the following corollary.

\begin{corollary}
\label{cor:delta-reg-iff-exists-M-b}
    There exists an $k$-dimensional affine subspace $\calU$ for which $f_\calU$ is $\delta$-regular if and only if there exists an invertible $M: \F_2^n \rightarrow \F_2^n$ and a fixing of the last $n-k$ coordinates, $b\in \F_2 ^{\overline{[k]}}$ such that $\Restricted{f\circ M}{\overline{[k]}}{b}$ is $\delta$-regular.
\end{corollary}

We use \Cref{cor:delta-reg-iff-exists-M-b} crucially in the proof of \Cref{thm:bounded-deg-d-upper-bound-intro}, wherein we construct $M$ and $b$ such that $\Restricted{f\circ M}{\overline{[k]}}{b}$ has small Fourier coefficients.
In the proof of the Theorem we will also need to understand the Fourier coefficients of $f\circ M$ in terms of the Fourier coefficients of $f$. The following fact, gives an identity between the Fourier coefficients of the two functions. 

%Finally, we give a way to compute the Fourier coefficients of $f_{\alpha + \calV}$ in terms of the old Fourier coefficients of $f$. Towards this end, the following fact will be useful.
\begin{fact}[\cite{AOBFbook}, Exercise 3.1]

\label{fact:fourier-coeffs-linear-transformation}

Let $M$ be an invertible linear transformation, and consider the function $g = f \circ M: \F_2^n \to \R$. Then we have that

$$\hat{g}(\gamma) = \hat{f}(M^{-\transpose} \gamma).$$

\end{fact}
%For completeness, we include the proof.
\begin{proof}
We have that
\begin{align*}
    \hat{g}(\gamma) = \E_x[g(x) \chi_\gamma(x)] &= \E[f(Mx) \chi_\gamma(x)] \\
    &= \E_y[f(y) \chi_\gamma(M^{-1}y)] \\
    &= \E_y[f(y) \chi_{M^{-\transpose}\gamma}(y)] = \hat{f}(M^{-\transpose} \gamma),
\end{align*}
where we have used the fact that $\chi_\gamma(M^{-1}y) = (-1)^{\inner{\gamma,M^{-1} y}} = (-1)^{\inner{M^{-\transpose}\gamma, y}}$. 
\end{proof}

Lastly, we see how the Fourier coefficients of $f_\calU$ can be written in terms of the Fourier coefficients of $f$. It turns out that we can associate the characters with affine subspaces of $\calV^{\perp}$ and express Fourier coefficient of a character as signed sum of the Fourier coefficients of $f$ coming from the corresponding affine subspace. This view of the Fourier coefficients under restrictions will be useful for us when we construct functions and argue that their regularity numbers must be large. 

\begin{fact}
\label{fact:Fourier-coeff-of f_U-as-a-sum-of-fourier-coeff-of-f-from-vperp}
Let $\calU =\alpha+\calV$ be an affine subspace of $\calV$. There is an isomorphism $L : \hat \calV \to \F_2^n/\calV^\perp$ and using this isomorphism, we can write 
    $$\hat{f_{\calU}}(\chi) = \sum_{\eta \in L\rchi} \hat{f}(\eta)(-1)^{\inner{\eta, \alpha}}$$
    for any $\chi \in \hat{\calV}$.
\end{fact}

\begin{proof}
For a complement space $\calW$ of $\calV^{\perp}$, from \Cref{fact:coefficients-as-expectation} we get an invertible linear map $R:\hat{\calV}\to \calW$ and denoting $\gamma := R\rchi$ we can write
\begin{align*}
\hat{f_{\calU}}(\chi)  = (-1)^{\inner{\gamma,\alpha}}\E_{x\in \calU}[f(x)(-1)^{\inner{\gamma,x}}] &= \E_{y\in \calV}[f(y+\alpha)(-1)^{\inner{\gamma,y}}] \\
&= \E_{y\in \calV}\left[\sum_{\beta\in \F_2^n}\hat{f}(\beta)(-1)^{\inner{\beta,y+\alpha}}(-1)^{\inner{\gamma,y}}\right] \\
&= \sum_{\beta\in \F_2^n}\hat{f}(\beta)(-1)^{\inner{\beta,\alpha}}\E_{y\in\calV}\left[(-1)^{\inner{\gamma+\beta,y}}\right] = \sum_{\eta\in \gamma+\calV^{\perp}}\hat{f}(\eta)(-1)^{\inner{\eta,\alpha}},
\end{align*}
which follows by observing that  $\E_{y\in\calV}\left[(-1)^{\inner{\gamma+\beta,y}}\right] = 1$ if $\beta\in \gamma+\calV^{\perp}$ and zero otherwise. Lastly, we note that  $\hat{\calV} \cong \calW\cong \F_2^n/\calV^{\perp}$ and the isomorphism $L$ is implicitly given by the above calculation. 
\end{proof}
% Letting $L$ be such a map, between $\hat{\calV}$ and $\F_2^n/\calV^{\perp}$, we can rewrite the above equation for every $\chi\in \hat{\calV}$ as
% $\hat{f_\calU}(\chi) = \sum_{\eta \in L\rchi} \hat{f}(\eta)(-1)^{\inner{\eta, \alpha}}.$

We have the following simple corollary.

\begin{corollary}
\label{cor:V-dim-n-1}
When $\calV$ has dimension $n-1$, this corresponds to fixing a single parity $\sum_{i: \gamma_i = 1}x_i$ to $b \in \{0,1\}$. Then $\calV^\perp$ is simply $\spn(\{\gamma\})$ and $\alpha$ is any vector such that $\inner{\gamma, \alpha} = b$. 

Then for all $\gamma' \neq \gamma$ we have by \Cref{fact:Fourier-coeff-of f_U-as-a-sum-of-fourier-coeff-of-f-from-vperp} that 
$$\hat{f_{\alpha + \calV}}(\chi_{\gamma'}) = (-1)^{\inner{\gamma', \alpha}}\hat{f}(\gamma') + (-1)^{\inner{\gamma + \gamma', \alpha}} = (-1)^{\inner{\gamma', \alpha}}\left (\hat{f}(\gamma') + (-1)^b\cdot \hat{f}(\gamma + \gamma')\right ).$$
In particular, there exists a choice of $b$ such that
$$\left |\hat{f_{\alpha + \calV}}(\chi_\mathbf{0})\right | =\left | \hat{f}(\mathbf{0}) + \hat{f}(\gamma)\right | .$$
\end{corollary}



